AdaMMS: Model Merging for Heterogeneous Multimodal Large Language Models with Unsupervised Coefficient Optimization

Recently, model merging methods have demonstrated powerful strengths in combining abilities on various tasks from multiple Large Language Models (LLMs). While previous model merging methods mainly focus on merging homogeneous models with identical architecture, they meet challenges when dealing with Multimodal Large Language Models (MLLMs) with inherent heterogeneous property, including differences in model architecture and the asymmetry in the parameter space. In this work, we propose AdaMMS, a novel model merging method tailored for heterogeneous MLLMs. Our method tackles the challenges in three steps: mapping, merging and searching. Specifically, we first design mapping function between models to apply model merging on MLLMs with different architecture. Then we apply linear interpolation on model weights to actively adapt the asymmetry in the heterogeneous MLLMs. Finally in the hyper-parameter searching step, we propose an unsupervised hyper-parameter selection method for model merging. As the first model merging method capable of merging heterogeneous MLLMs without labeled data, extensive experiments on various model combinations demonstrated that AdaMMS outperforms previous model merging methods on various vision-language benchmarks.

==> floats/avg5_gain.tex <==
\begin{table*}[!ht]
    \centering
       \resizebox{\textwidth}{!}{%      
    \begin{tabular}{lcccccccccc}
    \toprule
        \textbf{Model} & $\mathrm{MMMU_{val}}$ &  $\mathrm{MME_{sum}}$ &  $\mathrm{SeedBench_{all}}$ & $\mathrm{OCRBench}$  &  $\mathrm{TextVQA_{val}}$  & $\mathrm{OKVQA}$ & $\mathrm{GQA}$  &  $\mathrm{VizWiz_{val}}$ & $\mathrm{SUM}$ & $\mathrm{Top2}$ \\ 
        \midrule
        
       Task Arithmetic  & \underline{12.21}  & \textbf{19.27}  & \textbf{13.06}  & 0.50  & 1.10  & \underline{14.29}  & \underline{-3.61}  & \underline{-20.60}  & \underline{36.28} &7  \\ 
       
         Ties-Merging  & -1.92  & -22.34  & -27.69  & 3.80  & -23.86  & -18.49  & -29.04  & -37.32  & -156.80 &0 \\ 
         DARE-Linear  & 7.15  & -4.61  & 9.14  & -10.30  & -14.49  & 5.55  & -13.30  & -33.81  & -54.61 &0 \\ 
         DARE-Ties  & -11.53  & -55.63  & -7.05  & -44.30  & -38.43  & -19.88  & -24.80  & -42.54  & -244.12 & 0 \\ 
         MetaGPT  & 1.14  & -5.81  & -5.51  & \textbf{17.40}  & \underline{5.16}  & -6.09  & -24.07  & -30.21  & -47.94 &2 \\ 
         \textbf{AdaMMS}  & \textbf{14.38 } & \underline{15.21}  & \underline{10.17}  & \underline{15.30}  & \textbf{22.52 } & \textbf{15.00}  & \textbf{-1.39}  & \textbf{-13.60}  & \textbf{77.64} &9 \\ \hline

    \end{tabular}
    }
    \caption{Results of the performance gain among all model pairs.}
    \label{tab:avg}
\end{table*}

==> floats/llava2cog-alpha.tex <==

\begin{table*}[!ht]
    \centering
    \small
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{cccccccccc}
    \toprule
          Model & $\mathrm{MMMU_{val}}$ &  $\mathrm{MME_{sum}}$ &  $\mathrm{SeedBench_{all}}$ & $\mathrm{OCRBench}$  &  $\mathrm{TextVQA_{val}}$  & $\mathrm{OKVQA}$ & $\mathrm{GQA}$  &  $\mathrm{VizWiz_{val}}$ & $\mathrm{SUM}$    \\ 
        
          \hline
\rowcolor{gray!20}
\multicolumn{10}{c}{\textbf{Original Models}} \\
\hline
         CogVLM\footnotesize(base) & 34.80 & 59.23 & 61.22 & 56.50 & 77.57 & 60.82 & 59.43 & 37.09 & 446.66 \\ 
        LLaVA & 35.10 & 66.68 & 60.52 & 31.30 & 46.04 & 53.42 & 61.94 & 54.29 & 409.29 \\ 
        AVG & 34.95 & 62.96 & 60.87 & 43.90 & 61.81 & 57.12 & 60.69 & 45.69 & 427.98 \\ 
     
          \hline
\rowcolor{gray!20}
\multicolumn{10}{c}{\textbf{Linear Interpolation}} \\
\hline
        $\alpha$-0.1 & 34.90 & 63.32 & 62.97 & \textbf{57.00} & \textbf{76.90} & 61.11 & 60.12 & 37.09 & 453.41 \\ 
        $\alpha$-0.2 & 36.10 & 66.24 & 64.49 & 56.70 & 75.37 & 62.04 & 59.92 & \textbf{37.40} & 458.26 \\ 
        $\alpha$-0.3 & 36.70 & 69.09 & 65.65 & 55.70 & 73.34 & 62.53 & 59.46 & 37.27 & 459.74 \\ 
        $\alpha$-0.4 &\textbf{ 37.20} & \textbf{69.56} & \textbf{66.15} & 53.30 & 71.26 & \textbf{62.87} & 58.56 & 36.81 & 455.71 \\ 
        $\alpha$-0.5 & 36.70 & 66.01 & 65.98 & 51.30 & 68.90 & 61.96 & 58.92 & 35.73 & 445.50 \\ 
        $\alpha$-0.6 & 35.70 & 67.00 & 64.12 & 47.00 & 64.53 & 60.18 & \textbf{60.23} & 35.59 & 434.35 \\ 
        $\alpha$-0.7 & 34.30 & 59.48 & 59.79 & 40.80 & 57.60 & 56.34 & 56.73 & 33.08 & 398.12 \\ 
        $\alpha$-0.8 & 29.80 & 36.37 & 46.75 & 31.30 & 43.42 & 41.04 & 43.44 & 23.77 & 295.89 \\ 
          \hline
\rowcolor{gray!20}
\multicolumn{10}{c}{\textbf{Our Method}} \\
\hline

        AdaMMS & 34.9 & 69.09 & 64.12 & 55.7 & 76.9 & 61.11 & 60.12 & 37.27 & 459.21 \\ 
        Selceted a & 0.1 & 0.3 & 0.6 & 0.3 & 0.1 & 0.1 & 0.1 & 0.3 & - \\
        Distance with the best $\alpha$ & 0.3 & 0.1 & 0.2 & 0.2 & 0 & 0.3 & 0.5 & 0.1 & - \\
        \bottomrule
    \end{tabular}
    }
    \caption{Candidate linear interpolation results for AdaMMS and the $\alpha$ selected by our unsupervised hyper-parameter selection method on merging CogVLM-7B into LLaVA-v1.5-7B. AVG shows the average performance of the two original models.}
    \label{tab:inter_alpha}
\end{table*}

==> floats/llava2sharegpt.tex <==

\begin{table*}[!ht]
    \centering
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{llllllllll}
    \toprule
     \textbf{Model} & $\mathrm{MMMU_{val}}$ &  $\mathrm{MME_{sum}}$ &  $\mathrm{SeedBench_{all}}$ & $\mathrm{OCRBench}$  &  $\mathrm{TextVQA_{val}}$  & $\mathrm{OKVQA}$ & $\mathrm{GQA}$  &  $\mathrm{VizWiz_{val}}$ & $\mathrm{SUM}$ \\ 
        \midrule
     0.0(Sharegpt) & 36.60  & 65.32  & 63.72  & 37.60  & 46.88  & 50.98  & 63.27  & 60.38  & 424.75  \\ 
        0.1 & 36.20  & 65.94  & 63.77  & 37.70  & 47.11  & 52.31  & 63.35  & 60.30  & 426.68  \\ 
        0.2 & 36.90  & 66.32  & 63.73  & 37.40  & 47.28  & 53.78  & 63.40  & 60.55  & 429.36  \\ 
        0.3 & 35.80  & 67.13  & 63.42  & 37.30  & 47.42  & 54.14  & 63.44  & 60.42  & 429.07  \\ 
        0.4 & 36.20  & 67.20  & 63.29  & 37.20  & 47.60  & 54.51  & 63.29  & 59.85  & 429.14  \\ 
        0.5 & 36.40  & 67.63  & 63.39  & 37.20  & 47.58  & 54.60  & 63.13  & 59.37  & 429.30  \\ 
        0.6 & 37.10  & 67.20  & 63.22  & 36.80  & 47.28  & 54.65  & 62.95  & 59.18  & 428.38  \\ 
        0.7 & 37.00  & 66.51  & 63.10  & 36.70  & 46.93  & 54.67  & 62.77  & 58.64  & 426.32  \\ 
        0.8 & 36.30  & 66.24  & 62.95  & 36.50  & 46.78  & 54.53  & 62.70  & 58.10  & 424.10  \\ 
        0.9 & 36.30  & 66.48  & 62.72  & 35.60  & 46.44  & 53.82  & 62.57  & 57.41  & 421.34  \\ 
        1.0(LLaVA) & 34.90  & 67.42  & 62.20  & 34.60  & 46.04  & 53.05  & 62.32  & 56.81  & 417.34  \\ 
        Task Arithmetic  & 36.10  & 69.61  & 63.40  & 37.00  & 50.65  & 53.37  & 63.13  & 59.29  & 432.55  \\ 
        Ties-Merging  & 35.90  & 69.57  & 61.73  & 35.70  & 50.36  & 54.44  & 63.17  & 54.89  & 425.76  \\ 
        DARE-Linear  & 36.30  & 69.40  & 63.36  & 37.40  & 50.70  & 53.71  & 63.06  & 59.55  & 433.48  \\ 
        DARE-Ties  & 32.80  & 58.59  & 56.49  & 32.60  & 44.11  & 50.20  & 57.23  & 43.78  & 375.80  \\ 
        MetaGPT & 36.30  & 70.58  & 63.44  & 37.10  & 50.93  & 53.57  & 63.23  & 59.72  & 434.87  \\ 
        diff3-sample0.1-EM & 36.30  & 66.48  & 63.77  & 37.30  & 47.60  & 54.14  & 63.13  & 60.55  & 429.27 \\ 
        \bottomrule
    \end{tabular}%
        }
    \caption{Results on various benchmark when merging LLaVA-v1.5-7B into ShareGPT-4V-7B.}
     \label{tab:llava2share}

\end{table*}

==> floats/qwen0.02.tex <==

\begin{table}[!ht]
    \centering
    \begin{tabular}{llll}
     \toprule
        \textbf{Model} & $\mathrm{MMMU_{val}}$ &  $\mathrm{MME_{sum}}$ & $\mathrm{OCRBench}$   \\ 
        \midrule
       
        alpha-0.00 & 50.11  & 81.44  & \textbf{86.00}  \\ 
        alpha-0.02 & 49.67 & 81.69  & \textbf{86.00}  \\ 
        alpha-0.04 & 50.00  & 80.96  & 85.50  \\ 
        alpha-0.06 & 49.89  & 81.13  & 85.30  \\ 
        alpha-0.08 & 49.33  & 81.32  & 85.50  \\ 
        alpha-0.10 & 50.56  & 81.46  & 85.50  \\ 
        alpha-0.12 & 50.11  & 81.92  & 85.70  \\ 
        alpha-0.14 & 50.78  & 82.39  & 85.70  \\ 
        alpha-0.16 & 50.44  & 82.05  & 85.70  \\ 
        alpha-0.18 & 51.00  & 83.02  & 85.40  \\ 
        alpha-0.20 & 51.11  & 82.36  & 85.20  \\ 
        alpha-0.22 & 50.11  & 83.37  & 85.30  \\ 
        alpha-0.24 & 51.11  & 82.72  & 85.00  \\ 
        alpha-0.26 & 51.11  & 82.80  & 84.70  \\ 
        alpha-0.28 & 51.11  & \textbf{83.63}  & 84.40  \\ 
        alpha-0.30 & \textbf{51.22}  & 83.36  & 84.40  \\ 
        alpha-0.32 & 51.00  & 83.47  & 83.90  \\ 
        alpha-0.34 & 50.33  & 83.48  & 83.10  \\ 
        alpha-0.36 & 50.22  & 83.22  & 82.10  \\ 
        alpha-0.38 & 50.00  & 82.96  & 81.30  \\ 
        alpha-0.40 & 50.67  & 83.03  & 80.70  \\ 
        alpha-0.42 & 50.11  & 83.37  & 79.80  \\ 
        alpha-0.44 & 49.89  & 83.02  & 78.90  \\ 
        alpha-0.46 & 49.78  & 83.13  & 78.20  \\ 
        alpha-0.48 & 48.89  & 82.57  & 77.30  \\ 
        alpha-0.50 & 50.00  & 81.37  & 76.40 \\ 
          \midrule
        diff3-EM  & 50.44 & 83.42 &85.30 \\
         \bottomrule
    \end{tabular}%
    % }
    \caption{Results on 0.02 interval. }
    \label{tab:qwen0.02}
\end{table}

==> floats/qwen0.05.tex <==

\begin{table}[!ht]
    \centering
    % \resizebox{\textwidth}{!}{%
    \begin{tabular}{lccc}
        \toprule
        {Model} & $\mathrm{MMMU_{val}}$ &  $\mathrm{MME_{sum}}$ & $\mathrm{OCRBench}$   \\ 
        \midrule
        \(\alpha\)-1.00 & 50.11  & 81.44  & \textbf{86.00}  \\ 
        \(\alpha\)-0.95 & 49.67  & 81.24  &  85.50 \\ 
        \(\alpha\)-0.90 & 50.56  & 81.46  & 85.50  \\ 
        \(\alpha\)-0.85 & 50.67  & 82.79  & 85.50  \\ 
        \(\alpha\)-0.80 & 51.11  & 82.36  & 85.20  \\ 
        \(\alpha\)-0.75 & 51.11  & 82.88  & 84.60  \\ 
    \(\alpha\)-0.70 & \textbf{51.22}  & 83.36  & 84.40  \\ 
        \(\alpha\)-0.65 & 50.33  & 83.12  & 82.80  \\ 
        \(\alpha\)-0.60 & 50.67  & 83.03  & 80.70  \\ 
        \(\alpha\)-0.55 & 49.33  & \textbf{83.26}  & 79.00  \\ 
        \(\alpha\)-0.50 & 50.00  & 81.37  & 76.40  \\ 
        \(\alpha\)-0.45 & 47.78  & 81.40  & 74.30  \\ 
        \(\alpha\)-0.40 & 47.00  & 82.06  & 71.20 \\
          \midrule
    Oracle\footnotesize(Upper Bound) & 51.22\footnotesize(0.70) & 83.36\footnotesize(0.70) & 85.50\footnotesize(0.10) \\   
       \ours &   51.11\footnotesize(0.80)  & 83.36\footnotesize(0.70)  &  85.50\footnotesize(0.10) \\
     \bottomrule
    \end{tabular}%
    % }
    \caption{Results on0.05 interval. }
    \label{tab:qwen0.05}
\end{table}

==> floats/supervised.tex <==
\begin{table*}[!ht]
    \centering
     \resizebox{\textwidth}{!}{
    \begin{tabular}{lllllllllll}
    \hline
        Model & MMMU\_val & MME\_sum & Seed-Bench\_all & OCRBench & TextVQA\_val & OK-VQA & GQA & VizWiz\_val & Sum & Again  \\ \hline
        AdaMMS & 34.90  & 69.09  & 64.12  & 55.70  & 76.90  & 61.11  & 60.12  & 37.27  & 459.21  & +31.23 \\ 
        Ties-Merging  & 34.00  & 57.29  & 38.97  & 55.00  & 59.73  & 40.31  & 51.97  & 24.36  & 361.63  & -66.35 \\ 
        Ties-Merging(supervised) & 37.20  & 57.29  & 63.12  & 55.90  & 76.50  & 61.45  & 55.81  & 37.98  & 445.25  & +17.27 \\ 
        Ties-Merging(optimal) & 37.20  & 63.96  & 65.43  & 55.90  & 76.55  & 61.45  & 57.99  & 38.21  & 456.69  & +28.71 \\ \hline
    \end{tabular}}
    \label{supervised}
\end{table*}
